Deep MMD Gradient Flow without adversarial training

We propose a gradient flow procedure for generative modeling by transporting particles from an initial source distribution to a target distribution, where the gradient field on the particles is given by a noise-adaptive Wasserstein Gradient of the Maximum Mean Discrepancy (MMD). The noise-adaptive MMD is trained on data distributions corrupted by increasing levels of noise, obtained via a forward diffusion process, as commonly used in denoising diffusion probabilistic models. The result is a generalization of MMD Gradient Flow, which we call Diffusion-MMD-Gradient Flow or DMMD. The divergence training procedure is related to discriminator training in Generative Adversarial Networks (GAN), but does not require adversarial training. We obtain competitive empirical performance in unconditional image generation on CIFAR10, MNIST, CELEB-A (64 x64) and LSUN Church (64 x 64). Furthermore, we demonstrate the validity of the approach when MMD is replaced by a lower bound on the KL divergence.

==> intro_old.tex <==


% Consider a space $\mathcal{X} \in \rset^{D}$ and a set $\mathcal{P}(\mathcal{X})_{2}$ of probability distributions defined on $\mathcal{X}$. Let $P \in \mathcal{P}(\mathcal{X})$ and $Q \in \mathcal{P}(\mathcal{X})$ are two distributions defined on $\mathcal{X}$. We call $P$ the \textit{source} probability distribution and $Q$ the \textit{target} one.

% Assume that we have samples $X^N = \{ x_i \}_{i=1}^{N} \sim P(X)$ from the \textit{source} distribution and the samples $Y^M = \{ y_i \}_{i=1}^{M} \sim Q(Y)$ from the \textit{target} one. We are interested in solving two problems. First, we want to build a \textbf{discriminator} $\mathcal{D}$ which can accurately distinguish samples from the source and the target distribution. Second, we aim to find a mapping which can transform the samples from the source distribution to the target one.

% Both problems presented above can be solved using Generative Adversarial Networks (GANs) \citep{} which have many variants (see \citep{}). However, GAN approach requires to use adversarial training \citep{}.

% If we are interested only in transforming samples from a source to a target distribution, recently many techniques were developed which include Flow Matching \citep{}, Shrodinger Bridges \citep{}, as well as Diffusion Models \citep{}. Diffusion models will be applicable if the source distribution $P(X) = \mathrm{N}(0, \Id)(X)$.

% If we assume that we already have a discriminator $\mathcal{D}$ and we can define a Wasserstein Gradient Flow \citep{} of it, then we can use the gradient flow to transform samples from source to target. The gradient flow needs to be well defined and depends on the discriminator function.

% In this paper, we propose an approach which allow to train a discriminator without requiring the adversarial training which is used in GANs. On top of that, we propose a method based on the Wasserstein Gradient Flow which could use the trained discriminator to produce samples from the distribution of interest. Our approach combines the ideas from regularizing the GAN discriminator training as well as the ideas from the diffusion models allowing to produce noisy version of samples for the given level of noise $t$. We demonstrate the empirical effectiveness of the method and provide the theoretical guarantees.

% \valentin{Introduction quite good but a bit too long and might be fleshed out. Some repetition in the part about the flow of GAN}

In  recent years, generative models have achieved impressive capabilities on image \cite{saharia2022photorealistic}, audio \cite{le2023voicebox} and video generation \cite{ho2022imagen} tasks but also protein modeling \cite{watson2022broadly} and 3d generation \cite{poole2022dreamfusion}. Diffusion models \citep{sohldickstein2015deep,ho2020denoising,song2020score,rombach2022highresolution} underpin many of these new methods. In these models, we learn a backward denoising diffusion process via denoising score matching~\citep{hyvarinen05a,vincent11}. This backward process corresponds to the time-reversal of a forward noising process. At sampling time, starting from random noise, diffusion models produce samples by discretizing the backward sampling process. 

%Doing so, one can leverage fine-grained control sampling strategies like improved samplers \cite{zhang2022fast} or predictor-corrector schemes \cite{song2020score}. 
% Diffusion models however, could suffer from convergence problems on sub-manifolds~\citep{debortoli2023convergence} as the samples in the backward diffusion process approach the data. 
One challenge that arises when applying these models in practice is that the score (that is, the gradient log of the current noisy density) becomes ill-behaved for low noise levels, as we approach the data distribution~\citep{yang2023eliminating}. The diffusion process needs to be slowed down at this point, which incurs a large number of sampling steps near the data distribution. \textcolor{red}{Indeed, if the manifold hypothesis holds \cite{tenenbaum2000global,fefferman2016testing,brown2022union} and the data is supported on a lower dimensional space, it is expected that the score will explode for noise levels close to zero, to ensure that the backward process concentrates on this lower dimensional manifold \cite{debortoli2023convergence,pidstrigach2022score,chen2022sampling}.}  
While strategies exist to mitigate these issues, they all trade-off the quality of the output against inference speed, see~\citep{song2023consistency,xu2023ufogen,sauer2023adversarial} for instance. 
This puts diffusion models at one end of the spectrum with high quality of samples but long generation time. 

At the other end of the spectrum are Generative Adversarial Networks (GANs)~\citep{goodfellow2014generative}, which only require one forward pass to sample: hence, sample generation is very computationally efficient.
On the downside, samples are of lower quality samples than diffusion models~\citep{ho2020denoising,rombach2022highresolution}. 
% In the past years, however, GANs achieved strong performance~\citep{brock2019large,karras2020training} on many image generation tasks. 
Due to the adversarial nature of the objective function in GANs, they are notoriously difficult to train and require an extensive hyperparameter tuning~\citep{brock2019large,karras2020analyzing,liu2020generative}, may suffer from training instability and mode collapse~~\citep{arora2017generalization,kodali2017convergence,salimans2016improved}. Assuming that the training of a GAN is well tuned, the generator synthesizes samples which at start of the training are similar to random noise and as training progresses become more and more similar to samples from the target data distribution. At the same time, the discriminator also gradually improves a very coarse one, discriminating between data and random noise, to a very nuanced one, discriminating between samples close to the data and the data itself.
% \valentin{can you point me (maybe on gchat) to a reference talking about "weak" and "strong" discriminator. If anyone uses this terminology I won't argue with it but I find it weird.}
This process might converge to an equilibrium where the generator models the data distribution well, but this is not guaranteed in general~\citep{arora2017generalization}. 
% and besides choosing hyperparameters for GANs, we do not have much control over this.
% \ag{I think this last sentence is important for the next paragraph}
% \valentin{This sentence feels a bit redundant compared to what you said before. What point are you trying to make with that sentence}.
While using a generator in a GAN gives a fast way to sample data, it also does not give us control over the sampling process, besides modifying the random noise passed to the generator~\citep{arbel2021generalized,che2021gan,ansari2021refining}.
% Moreover, while the one-step generation process of GANs might seem like an advantage, it also does not give us much control over this sampling process besides modifying the random noise passed to the generator~\citep{arbel2021generalized,che2021gan,ansari2021refining}.
% \valentin{in fact here something that would have been interesting is to do a version of conditional guidance for MMDflow, since this is clearly not possible for GAN... Too late however but keep the idea}

% \ag{Valentin, can you please take a look?}
% In the past years, GANs achieved strong performance~\citep{brock2019large,karras2020training} on many image generation tasks, but were recently surpassed by diffusion models~\citep{ho2020denoising,rombach2022highresolution}. Due to the adversarial nature of the objective function in GANs, they are notoriously difficult to train and require an extensive hyperparameter tuning~\citep{brock2019large,karras2020analyzing,liu2020generative}, may suffer from training instability and mode collapse~~\citep{arora2017generalization,kodali2017convergence,salimans2016improved}. Assuming that the training of a GAN is well tuned, the generator produces samples which at start of the training look like random noise and as training progresses look similar to the data. At the same time, the discriminator also gradually improves from the weak one, discriminating between data and random noise, to a strong one, discriminating between samples close to the data and the data itself. This process might converge to an equilibrium where generator models well the data distribution, but this is not guaranteed in general~\citep{arora2017generalization} and besides choosing hyperparameters for GANs, we do not have much control over this. \valentin{This sentence feels a bit redundant compared to what you said before. What point are you trying to make with that sentence}. Moreover, while the one-step generation process of GANs might seem like an advantage, it also does not give us much control over this sampling process besides modifying the random noise passed to the generator~\citep{arbel2021generalized,che2021gan,ansari2021refining}.



% The drawback of these models is that naive implementations require many denoising steps to generate samples. While many improvements~\citep{zhang2022fast,song2020score} have been proposed, an alternative approach is to use Generative Adversarial Networks (GANs)~\citep{goodfellow2014generative}. \valentin{Do we want to sell our method as a faster way of doing diffusion models? We don't really have experiments to showcase this} In GANs, we train a generator and a discriminator using adversarial training objective. GANs require only one sampling step at inference time compared to diffusion models which makes them a faster alternative. The drawback, however, is the lack of control over the sampling process unlike in diffusion models.
% \valentin{We can keep going back and forth between. GANs go fast. GANs give bad quality (cf next sentence as well). I would rephrase this first paragraph to focus on diffusion models. Then next paragraph. Just say once: diffusion models are at one end of the spectrum with long generation time but high quality. GANS are at the other end of the spectrum with extremely fast generation but usually not good. GANs suffer from other problems as well (i.e. adversarial training). Our goal? Improve GAN training and sampling with ideas from diffusion models}


% \ag{Especially this} Diffusion models however, could suffer from convergence problems on sub-manifolds~\citep{debortoli2023convergence} as the samples in the backward diffusion process approach the data. This is due to the ill-behaved score function~\citep{yang2023eliminating}. The implication in practice is the need to do many small sampling steps when approaching the data, which can significantly slow down the diffusion sampling process.



% \ag{Valentin, can you please take a look?}
% Diffusion models~\citep{sohldickstein2015deep,ho2020denoising,rombach2022highresolution} are currently SOTA on image generation tasks. In diffusion models, starting from the noisy version of the data produced from the forward diffusion process~\citep{ho2020denoising}, we train a backward diffusion process via conditional score matching~\citep{hyvarinen05a}. At sampling time, starting from random noise, diffusion models produce samples by using an iterative sampling procedure. This has an advantage of being able to use fine-grained control sampling strategies like improved samplers \cite{zhang2022fast} or predictor-corrector schemes \cite{song2020score}.
% \ag{Especially this} Diffusion models however, could suffer from convergence problems on sub-manifolds~\citep{debortoli2023convergence} as the samples in the backward diffusion process approach the data. This is due to the ill-behaved score function~\citep{yang2023eliminating}. The implication in practice is the need to do many small sampling steps when approaching the data, which can significantly slow down the diffusion sampling process.
% \valentin{I feel like this could go before the paragraph on GANs. I think a structure like this would make sense. Generative models is very cool (your current first paragraph). This is powered by diffusion models (this paragraph) but they have problems (they are at one end of the spectrum I was referring to before) (this paragraph too). On the other end of the spectrum we have GANs which are blazingly fast but not good generation (the previous paragraph)}



% At sampling time, we can have a fine-grained control sampling strategies like improved samplers \cite{zhang2022fast} or predictor-corrector schemes \cite{song2020score}. Diffusion models however, could suffer from convergence problems on sub-manifolds~\citep{debortoli2023convergence} as the samples in the backward diffusion process approach the data. This is due to the ill-behaved score function~\citep{yang2023eliminating}. The practical implication is the need to do many small steps near the data, which can significantly slow down the diffusion sampling process.

% GANs are notoriously difficult to train and require an extensive hyperparameter tuning~\citep{brock2019large,karras2020analyzing,liu2020generative}. Due to the adversarial nature of the loss, it is necessary to ensure that the discriminator and generator improve roughly at the same rate. On top of that, GANs may exhibit a mode collapse~\citep{arora2017generalization,kodali2017convergence}, a situation where 

% On top of that, training a GAN discriminator typically require heavy regularisations such as $\ell_2$ penalty~\citep{binkowski2021demystifying}, gradient penalty~\citep{gulrajani2017improved}, spectral normalization~\citep{miyato2018spectral}. GANs may exhibit a mode collapse \ag{add citation and an explanation why mode collapse is happening}.  % Finally, unlike in diffusion models where we can have a fine-grained control over sampling process, in GANs, we only rely on a fixed generator.

% DIFFUSIONS.\ag{Moreover, as the backward diffusion processs approaches the data, the score function becomes ill-behaved~\citep{yang2023eliminating}, which requires to do many small steps as we approach the data. All this makes the sampling procedure in diffusions slow.}

% \ag{Comment please on the structure of this paragraph}
Leveraging insights from both GANs and diffusion models, our contributions are two-fold. First, we propose a method to train a GAN-like discriminator which does not rely on adversarial training. Given clean data, we use a forward diffusion process from \citep{ho2020denoising} to produce a noisy version of the data with a given level of noise. Drawing inspiration from GAN training, the data with the high level of noise is analogous to the output of a poorly trained generator, whereas the data with the low level of noise would correspond to a well trained generator. 
% \valentin{Maybe this sentence could be skipped. Can keep for now}.
For a given level of noise, we train a noise conditional discriminator to distinguish between the clean and the noisy data. This allows us to have a fine grained control over the discriminator training procedure. As a discriminator, we use Maximum Mean Discrepancy (MMD)~\citep{gretton12a} since it is well-defined on distributions without overlapping support contrary to f-divergence~\citep{nowozin2016fgan} based discriminators. 

We propose a novel noise-adaptive version of MMD gradient flow~\citep{arbel2019maximum} to sample from the data distribution. We start from samples drawn from a Gaussian distribution, and move them in the direction of the target distribution by following MMD Gradient flow~\citep{arbel2019maximum} with a neural feature-parametrized MMD critic adapted to the corresponding  level of noise,  from  highest (source) to  lowest (target).
% Starting from a sample from Gaussian distribution, we follow the MMD gradient flow~\citep{arbel2019maximum} with a controlled level of noise, starting from the highest and going to the lowest noise level.
This allows us to have a fine grained control over the sampling process. We provide theoretical justification for the benefit of using adaptive kernel during the MMD gradient flow procedures. On top of that, we propose a scalable approximate sampling procedure for a case of a linear base kernel. Finally, we show that our method, Diffusion-MMD-gradient flow or \DMMD \ yields competitive performance in generative modeling in simple 2-D datasets as well as in unconditional image generation on CIFAR10~\citep{krizhevsky2009learning}.

% Starting from Gaussian noise and high level of noise, we foll

% without adversarial training, which is then later used in an adaptive Wasserstein gradient flow~\citep{ambrosioGradientFlowsMetric2008} to produce samples. Given clean data, we use a forward diffusion process from \citep{ho2020denoising} to produce a noisy version of the data with a given level of noise. Making the parallel with GAN training, the data with the high level of noise would correspond to a poorly trained generator whereas the data with the low level of noise would correspond to a well trained generator. For the given level of noise, we then train a noise conditional discriminator to distinguish between the clean and the noisy data.

% As a discriminator, we use Maximum Mean Discrepancy (MMD)~\citep{gretton12a} since it has nice property of being well define on distributions without overlapping support. Similar discriminator was used in MMD-GAN~\citep{binkowski2021demystifying,li2017mmd}. We regularize the training of a discriminator by using insights from GAN literature such as  $\ell_2$ penalty~\citep{binkowski2021demystifying} and gradient penalty~\citep{gulrajani2017improved} in order to stabilize the training. The resulted method therefore allows to train a GAN-like discriminator without adversarial training. At inference time, starting from the highest noise level, we follow MMD gradient flow~\citep{arbel2019maximum} gradually decreasing the noise level. This allows us to have fine grained control over the sampling process, similar to what could be done with diffusion models. Empirically, we show that the proposed method yields competitive performance in generative modeling of simple 2d toy datasets as well as on unconditional image generation on CIFAR10~\citep{krizhevsky2009learning}. The method enjoys similar convergence properties as described in \citep{arbel2019maximum}.

% In this paper, we propose a method to train a discriminator without adversarial training which is then later used in an adaptive gradient flow to produce samples. Our approach is inspired by the recent success of diffusion models. Given clean data, we generate noisy version of data using a  forward diffusion process then train a noise-conditional discriminator on top of this data. We regularize the training of a discriminator by using insights from GAN literature such as  $\ell_2$ penalty~\citep{binkowski2021demystifying} and gradient penalty~\citep{gulrajani2017improved} in order to stabilize the training. 
% \valentin{I have commented the following paragraph which is interesting but maybe too detailed for the introduction}
% % This learning algorithm for the discriminator mimics GAN training in a way that a discriminator for a high level of noise will be coarser/weaker whereas a discriminator for a low level of noise will be more detailed / stronger. In GAN training this effect happens during training a generator and a discriminator where initially both discriminator and generator are weak and then both become stronger. Later, we use this trained noise-conditional discriminator to generate samples using noise-adaptive gradient flow. 
% At inference time, starting from the highest noise level, we follow a gradient flow gradually decreasing the noise level. This allows us to have a fine grained control over the sampling process similar to diffusion model. Empirically, we show that the method yields \ag{strong} \valentin{alternative word would be "competitive"} performance in generative modeling of simple 2d toy datasets as well as of for generation tasks on image datasets such as CIFAR-10. The method relies on MMD gradient flow~\citep{arbel2019maximum} and therefore enjoys theoretical convergence properties of the generation process.

% The gradient flows can be used without adversarial training to generate samples, but they have 

% The main limitation of this approach, however, is the need for a discriminator. In practice, a common strategy is to use a handcrafted discriminator~\citep{arbel2019maximum,hertrich2023generative} optionally using pretrained features~\citep{li2024error}. Other strategy is to use adversarial training like in GANs either by training a normal GAN~\citep{ansari2021refining} or by replacing a generator by a gradient flow~\citep{franceschi2023unifying}. \ag{check if it reads better} These strategies, however, still rely on adversarial training and therefore may suffer from the same problems as GAN training.

% A different approach to generating samples could rely on a gradient flow from a discriminator, see \citep{arbel2019maximum,franceschi2023unifying}. In this setting, given a discriminator, one would sample particles from a source distribution (such as Gaussian Noise) and then move the particles in the direction of a gradient of discriminator. For some classes of discriminators, such as for example Maximum Mean Discrepancy (MMD)~\citep{gretton12a}, this approach is guaranteed to converge under some mild assumptions (see \citep{arbel2019maximum}). This means that the particles which were moved in the direction of a gradient flow, will have the same distribution as the target distribution which corresponds to a distribution we want to sample from. A nice property of gradient flow samplers is the ability to control sampling process by choosing discretisation schema, discretisation step and added noise, see \citep{arbel2019maximum}. The main limitation of this approach is the need for the discriminator. In practice, people either use hand-crafted discriminator such as \citep{arbel2019maximum,hertrich2023generative} or use pre-trained features such as in \citep{li2024error}. Other attempts of learning discriminator features rely on GAN training~\citep{ansari2021refining} or by using adversarial training and replacing generator by samples from gradient flow~\citep{franceschi2023unifying}. \ag{check if it reads better}

% In this paper, we propose a method to train a discriminator without adversarial training which is then later used in an adaptive gradient flow to produce samples. Our approach is inspired by the recent success of diffusion models. Given clean data, we generate noisy version of data using a  forward diffusion process then train a noise-conditional discriminator on top of this data. We regularize the training of a discriminator by using insights from GAN literature such as  $\ell_2$ penalty~\citep{binkowski2021demystifying} and gradient penalty~\citep{gulrajani2017improved} in order to stabilize the training. 
% \valentin{I have commented the following paragraph which is interesting but maybe too detailed for the introduction}
% % This learning algorithm for the discriminator mimics GAN training in a way that a discriminator for a high level of noise will be coarser/weaker whereas a discriminator for a low level of noise will be more detailed / stronger. In GAN training this effect happens during training a generator and a discriminator where initially both discriminator and generator are weak and then both become stronger. Later, we use this trained noise-conditional discriminator to generate samples using noise-adaptive gradient flow. 
% At inference time, starting from the highest noise level, we follow a gradient flow gradually decreasing the noise level. This allows us to have a fine grained control over the sampling process similar to diffusion model. Empirically, we show that the method yields \ag{strong} \valentin{alternative word would be "competitive"} performance in generative modeling of simple 2d toy datasets as well as of for generation tasks on image datasets such as CIFAR-10. The method relies on MMD gradient flow~\citep{arbel2019maximum} and therefore enjoys theoretical convergence properties of the generation process.

% \ag{maybe add discussion on improving GANs samples... che2021gan,arbel2021generalized,ansari2021refining}

% The advantage of these models is the ability to generate samples in one step. The disadvantage is that they are harder to train due to the adversarial objective and so far have achieved worse performance than diffusion models. \valentin{give more details and references here. I think at least part of the discussion of the limitation of GANs and a small introduction to GAN gradient flow should go here.}

% In this paper, we propose an approach which is inspired by both, GANs and diffusion models. We train a discriminator which is required to distinguish between clean data samples and noisy samples for a given level of noise produced from the forward diffusion process, similarly to what is done with diffusion models. Using the insights from GANs litterature we employ discriminator regularisation strategies to be able to train the discriminator. The resulting method of training discriminator does not require any adversarial training. On top of that, we show that the discriminator can be used to generate samples by employing a discriminator gradient flow. We demonstrate strong empirical performance on simple 2d toy datasets as well as on image generation datasets. An important advantage of this approach is also a theoretical guarantee of convergence of the generation process to the samples of the target distribution.

% \valentin{In the rest of this paper ... (present quickly the different sections)}§

